Friction-Adaptive Stochastic Nonlinear Model Predictive Control for Autonomous Vehicles

This paper addresses the trajectory-tracking problem under uncertain road-surface conditions for autonomous vehicles. We propose a stochastic nonlinear model predictive controller (SNMPC) that learns a tire--road friction model online using standard automotive-grade sensors. Learning the entire tire--road friction model in real time requires driving in the nonlinear, potentially unstable regime of the vehicle dynamics, using a prediction model that may not have fully converged. To handle this, we formulate the tire-friction model learning in a Bayesian framework, and propose two estimators that learn different aspects of the tire--road friction. The estimators output the estimate of the tire-friction model as well as the uncertainty of the estimate, which expresses the confidence in the model for different driving regimes. The SNMPC exploits the uncertainty estimate in its prediction model to take proper action when the uncertainty is large. We validate the approach in an extensive Monte-Carlo study using real vehicle parameters and in CarSim. The results when comparing to various MPC approaches indicate a substantial reduction in constraint violations, as well as a reduction in closed-loop cost. We also demonstrate the real-time feasibility in automotive-grade processors using a dSPACE MicroAutoBox-II rapid prototyping unit, showing a worst-case computation time of roughly 40ms.

==> SMPCWithGPLearningJournal copy 2/tikzdefs.tex <==
\usetikzlibrary{narrow}
%\tikzset{>=narrow}

\pgfplotsset{compat=newest,
every outer x axis line/.append style={-narrow,line width=1pt},
every outer y axis line/.append style={-narrow,line width=1pt},
every outer z axis line/.append style={-narrow,line width=1pt},
every axis plot/.append style={line width=1pt},
every axis x label/.append style={at={(1,0)},anchor=north east,yshift=-3pt,xshift=3pt},
every axis y label/.append style={at={(0,1)},anchor=north east,rotate=-90,xshift=-3pt,yshift=4pt},
/pgf/number format/1000 sep={},
tick align={outside},
/pgf/number format/fixed,
scaled ticks = false,
legend/.append style={draw=none},
plot coordinates/math parser=false,
}



\pgfplotsset{trim axis right,
	tick label style={font=\footnotesize},
	title style={font=\footnotesize,align=center},
	label style={font=\footnotesize,align=center},
	legend style={font=\footnotesize}}

==> SMPCWithGPLearningJournal copy 2/tikzdefsdown.tex <==
\usetikzlibrary{narrow}
%\tikzset{>=narrow}

\pgfplotsset{compat=newest,
	every outer x axis line/.append style={-narrow,line width=1pt},
	every outer y axis line/.append style={-narrow,line width=1pt},
	every outer z axis line/.append style={-narrow,line width=1pt},
	every axis plot/.append style={line width=1pt},
	every axis x label/.append style={at={(0.5,0)},anchor=south,yshift=-30pt,xshift=0pt},
	every axis y label/.append style={at={(0,1)},anchor=north east,rotate=-90,xshift=-3pt,yshift=4pt},
	/pgf/number format/1000 sep={},
	tick align={outside},
	/pgf/number format/fixed,
	scaled ticks = false,
	legend/.append style={draw=none},
	plot coordinates/math parser=false,
}



\pgfplotsset{trim axis right,
	tick label style={font=\footnotesize},
	title style={font=\footnotesize,align=center},
	label style={font=\footnotesize,align=center},
	legend style={font=\footnotesize}}

==> SMPCWithGPLearningJournal copy 2/tikzdefsrot2.tex <==
\usetikzlibrary{narrow}
%\tikzset{>=narrow}

\pgfplotsset{compat=newest,
every outer x axis line/.append style={-narrow,line width=1pt},
every outer y axis line/.append style={-narrow,line width=1pt},
every outer z axis line/.append style={-narrow,line width=1pt},
every axis plot/.append style={line width=1pt},
every axis z label/.append style={at={(1,0)},anchor=north east,yshift=-3pt,xshift=4pt},
every axis y label/.append style={at={(0,1)}, anchor=south east,xshift=0pt,yshift=0pt},
/pgf/number format/1000 sep={},
tick align={outside},
legend/.append style={draw=none},
plot coordinates/math parser=false,
}

==> SMPCWithGPLearningJournal copy 2/tikzdefsrot3.tex <==
\usetikzlibrary{narrow}
%\tikzset{>=narrow}

\pgfplotsset{compat=newest,
every outer x axis line/.append style={-narrow,line width=1pt},
every outer y axis line/.append style={-narrow,line width=1pt},
every outer z axis line/.append style={-narrow,line width=1pt},
every axis plot/.append style={line width=1pt},
every axis x label/.append style={at={(1,0)},anchor=north east,yshift=-3pt,xshift=4pt},
every axis y label/.append style={at={(0,1)}, anchor=south east,xshift=0pt,yshift=18pt},
/pgf/number format/1000 sep={},
tick align={outside},
legend/.append style={draw=none},
plot coordinates/math parser=false,
}

==> SMPCWithGPLearningJournal copy 2/tikzlibrarynarrow.code.tex <==
\pgfarrowsdeclare{narrow}{narrow}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=8.705\pgfutil@tempdima
  \advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by 2.85\pgflinewidth
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{170}{10\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-170}{10\pgfutil@tempdima}}}
  \pgfpathclose
  \pgfusepathqfillstroke
}


==> SMPCWithGPLearningJournal copy 2/tikztrim.tex <==
	\pgfplotsset{plot coordinates/math parser=false}
		  \pgfplotsset{/tikz/every picture/.append style={trim axis left,trim axis right}}

==> tikzdefsrot2.tex <==
\usetikzlibrary{narrow}
%\tikzset{>=narrow}

\pgfplotsset{compat=newest,
every outer x axis line/.append style={-narrow,line width=1pt},
every outer y axis line/.append style={-narrow,line width=1pt},
every outer z axis line/.append style={-narrow,line width=1pt},
every axis plot/.append style={line width=1pt},
every axis z label/.append style={at={(1,0)},anchor=north east,yshift=-3pt,xshift=4pt},
every axis y label/.append style={at={(0,1)}, anchor=south east,xshift=0pt,yshift=0pt},
/pgf/number format/1000 sep={},
tick align={outside},
legend/.append style={draw=none},
plot coordinates/math parser=false,
}

==> tikzdefsrot3.tex <==
\usetikzlibrary{narrow}
%\tikzset{>=narrow}

\pgfplotsset{compat=newest,
every outer x axis line/.append style={-narrow,line width=1pt},
every outer y axis line/.append style={-narrow,line width=1pt},
every outer z axis line/.append style={-narrow,line width=1pt},
every axis plot/.append style={line width=1pt},
every axis x label/.append style={at={(1,0)},anchor=north east,yshift=-3pt,xshift=4pt},
every axis y label/.append style={at={(0,1)}, anchor=south east,xshift=0pt,yshift=18pt},
/pgf/number format/1000 sep={},
tick align={outside},
legend/.append style={draw=none},
plot coordinates/math parser=false,
}

==> tikzlibrarynarrow.code.tex <==
\pgfarrowsdeclare{narrow}{narrow}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=8.705\pgfutil@tempdima
  \advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by 2.85\pgflinewidth
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{170}{10\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-170}{10\pgfutil@tempdima}}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

